StreamLearner: Distributed Incremental Machine Learning on Event Streams: Grand Challenge

Today, massive amounts of streaming data from smart devices need to be analyzed automatically to realize the Internet of Things. The Complex Event Processing (CEP) paradigm promises low-latency pattern detection on event streams. However, CEP systems need to be extended with Machine Learning (ML) capabilities such as online training and inference in order to be able to detect fuzzy patterns (e.g., outliers) and to improve pattern recognition accuracy during runtime using incremental model training. In this paper, we propose a distributed CEP system denoted as StreamLearner for ML-enabled complex event detection. The proposed programming model and data-parallel system architecture enable a wide range of real-world applications and allow for dynamically scaling up and out system resources for low-latency, high-throughput event processing. We show that the DEBS Grand Challenge 2017 case study (i.e., anomaly detection in smart factories) integrates seamlessly into the StreamLearner API. Our experiments verify scalability and high event throughput of StreamLearner.

==> content/problemOld.tex <==
\section{Challenges and Goals}
\label{sec:challenges}

Machine Learning (ML) trains a model with a given set of training data, e.g., building clusters, and then applies the trained model to solve problems, e.g., classifying unknown events. Traditional ML is \emph{batch-oriented}, i.e., the model is trained in a first step with a fixed set of---well-chosen---training data and then applied to the problems, without being adapted at run-time. 

However, in many cases, models are not static. In the course of streaming data becoming available from sensors, models need to be dynamically adapted. That means, that new data is taken into account in the learned model, while old data ``fades out'' and leaves the model, as it becomes irrelevant. 

This can be modeled by a \emph{sliding window} over the incoming event streams: Events within the window are relevant for the model training, whereas events that fall out of the window become irrelevant and should not be reflected in the model any longer.

The challenge in doing so is to support incremental processing / stream learning. The model should not be re-built from scratch for every new window, but rather incrementally be updated with new data while old data is removed.

Another challenge in ML in streaming data is that data from different streams might lead to independent models. For instance, data captured in one production machine might not be suitable to train the model of another production machine. The challenge is to determine which independent models shall be built based on which data from which incoming event streams. Further, the question is how to route the corresponding events to the appropriate model? When these questions are solved, the identified machine learning models can be built in parallel.


==> content/related.tex <==
% can be merged into the first section
\section{Related Work}
\label{sec:related}

%What has been done in this area? I have no clue yet ;-)

A large body of research addresses incremental (or online) learning of ML models: there are incremental algorithms for support vector machines \cite{cauwenberghs2001incremental}, neural networks \cite{furao2007enhanced}, or Bayesian models \cite{wilson2010bayesian}.
With StreamLearner, these algorithms can be parallelized easily to process independent stream partitions.

There are many general-purpose systems for stream processing such as Apache Kafka \cite{kreps2011kafka}, Apache Flink \cite{carbone2015apache}, Apache Storm \cite{toshniwal2014storm}, Apache Spark Streaming \cite{zaharia2013discretized}. These systems can implement the StreamLearner API as well. However, we wanted to keep fine-grained control over system resources in this paper to test performance and scalability in isolation.


